Human Activity Recognition Using 3D Orthogonally-projected EfficientNet on Radar Time-Range-Doppler Signature

In radar activity recognition, 2D signal representations such as spectrogram, cepstrum and cadence velocity diagram are often utilized, while range information is often neglected. In this work, we propose to utilize the 3D time-range-Doppler (TRD) representation, and design a 3D Orthogonally-Projected EfficientNet (3D-OPEN) to effectively capture the discriminant information embedded in the 3D TRD cubes for accurate classification. The proposed model aggregates the discriminant information from three orthogonal planes projected from the 3D feature space. It alleviates the difficulty of 3D CNNs in exploiting sparse semantic abstractions directly from the high-dimensional 3D representation. The proposed method is evaluated on the Millimeter-Wave Radar Walking Dataset. It significantly and consistently outperforms the state-of-the-art methods for radar activity recognition.

==> Human Activity Recognition Using 3D Orthogonally-projected EfficientNet on Radar Time-Range-Doppler Signature (Version 5171)/snippets.tex <==
\begin{table}[htbp!]
\centering 
\caption{Results of 2D/3D ResNet/EfficientNet}
\resizebox{.95\columnwidth}{!}{

\begin{tabular}{c|c|ccc}
\hline 
\multirow{3}{*}{Model}& \multirow{3}{*}{\#Parameters}  & \multicolumn{3}{c}{Leave-$n$-antenna-out}  \\
& &\multicolumn{3}{c}{Test Accuracy (\%)} \\
& &$n=1$ & $n=2$ & $n=3$ \\
% $i$ &  $\hat{\mathcal{F}}_{i}$ & $\hat{H}_{i} \times \hat{W}_{i}$ & $\hat{C}_{i}$ & $\hat{L}_{i}$ \\
\hline 
2D ResNet && & &  \\
2D EfficientNet && & &  \\
3D ResNet & & &&  \\
3D EfficientNet && & &  \\
\hline
\end{tabular} \label{tab:results2d3d} 
}
\end{table}



%%%%

\begin{figure}  %子图加并列
\centering
\subfigure[Before]{
\begin{minipage}[b]{0.22\textwidth}
\includegraphics[width=1\textwidth]{fig/zz_plt.png} 
\end{minipage}
}
\subfigure[After]{
\begin{minipage}[b]{0.22\textwidth}
\includegraphics[width=1\textwidth]{fig/ori_plt.png}
\end{minipage}
}
\caption{Range Doppler Map Before/After Processing}
\end{figure}

%%%%% Table 
\begin{table}[htbp!]
\centering 
\caption{Results of Different Number of Non-local Blocks}
% \resizebox{.95\columnwidth}{!}{

\begin{tabular}{cc|cc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Model}} & \multicolumn{2}{|c}{Test Acc (\%)} \\
 &  & $50/50$ & $2/2$ \\
% \multicolumn{2}{c|} { Model } & top-1 & top-5 \\
\midrule
\midrule
\multirow{3}{*} { 3D ResNet-10 } 
& without &  &  \\
& pos. a &  &  \\
& pos. b &  &  \\
\midrule
\multirow{4}{*} { 3D EfficientNet-B0 } 
& without &  &  \\
& pos. a &  &  \\
& pos. b & &  \\
& pos. c & &  \\
\bottomrule
\end{tabular}

\label{tab:resultblocks} 
% }
\end{table}



%%%%

\subsection{Non-local}



%%%%% Table 
\begin{table}[htbp!]
\centering 
\caption{Results of Different Number of Non-local Blocks}
% \resizebox{.95\columnwidth}{!}{

\begin{tabular}{cc|cc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Model}} & \multicolumn{2}{|c}{Test Acc (\%)} \\
 &  & $50/50$ & $2/2$ \\
% \multicolumn{2}{c|} { Model } & top-1 & top-5 \\
\midrule
\midrule
\multirow{3}{*} { 3D ResNet-10 } 
& without &  &  \\
& 1-block &  &  \\
& 5-block &  &  \\
\midrule
\multirow{3}{*} { 3D EfficientNet-B0 } 
& without &  &  \\
& 1-block &  &  \\
& 5-block & &  \\
\bottomrule
\end{tabular}

\label{tab:resultblocks} 
% }
\end{table}



%%%
Generally, we average the results from $6$ independent random shuffle 50\%-50\% splits and $6$ leave-$2$-antenna-out splits on the proposed methods. For the leave-$2$-antenna-out splits,  all the inputs generated from certain $2$ antennas are left for testing while remaining samples  are utilized for training, and thus there are 
$\big(\begin{smallmatrix}
  2 \\
  4 
\end{smallmatrix}\big)=6$  
combinations in total. This approach aims to forbid the information from certain $2$ antennas. Thus, the testing results could partly reveal model performance on unknown FMCW or on FMCW with less antennas.

%%%%
Some et al. [,] utilise wearable radar sensor to detect hand gesture. Their sensor has limited sensing range, closes to the detected hand and validated on consistent background. Hence, the sensor generate relatively clean signals and minor noise elimination should be considered. On the contrary, human activity recognition relatively longer detection range and consequently massive unrelated objects would be involved during sensing. The noises would be revealed on the generated images and thus reduce classification accuracy of the models. Thus, non-local block is introduced to the proposed 3D networks tackle this situation. 

%%%
Inspired by non-local means filter [] for denoising, non-local [] could resolve long-range dependency between pixels with weights. Meanwhile, the utilized embedded Gaussian non-local is a generalized version of self-attention [], which could introduce attentional behavior for the network to focus more on useful areas
% , while neglecting noises. 
Furthermore, the method can naturally interpret temporal information because related components within a video might be presented with long distance and time interval, and the model could interpret their dependency [].  


%%%%
Following (the experiment results from) Wang et al. [], we insert the non-local blocks at relatively deep stages because high-stage non-local blocks consumes less GPU memory and they have similar information abstraction ability with shallow layers, which introduces similar performances. $\{1,5\}$-block non-local are inserted into position \emph{a} or \emph{b} in 3D ResNet-10 as shown in Table \ref{tab:resnet} and inserted into position \emph{a}, \emph{b} or \emph{c} in 3D EfficientNet-B0 as shown in Table \ref{tab:eff}.



%%%%

\begin{table}[htbp!]
\centering 
\caption{Results of Proposed Architectures}
\resizebox{.95\columnwidth}{!}{

\begin{tabular}{c|c|cc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{params} & \multicolumn{2}{c}{Test Acc (\%)} \\
% \multirow{3}{*}{Model}& \multirow{3}{*}{\#Parameters}  & \multicolumn{3}{c}{Leave-$n$-antenna-out}  \\
% & &\multicolumn{3}{c}{Test Accuracy (\%)} \\
 &  & $50/50$ & $2/2$ \\
% $i$ &  $\hat{\mathcal{F}}_{i}$ & $\hat{H}_{i} \times \hat{W}_{i}$ & $\hat{C}_{i}$ & $\hat{L}_{i}$ \\
\midrule
\midrule
2D ResNet-10 &   & &   \\
2D EfficientNet-B0 & & &  \\
\midrule
3D ResNet-10 & & &  \\
3D EfficientNet-B0  & & &  \\
\midrule
3D ResNet-10 + Non-local& & &  \\
3D EfficientNet-B0 + Non-local& & &   \\
\bottomrule
\end{tabular} \label{tab:results2d3d} 
}
\end{table}


%%%%
Radar signals are processed into time–range–Doppler data cube through range-Doppler processing \cite{li2019survey, liu2020real}. Some works further squeeze the cube into time-Doppler maps [?] or time-range [?] maps for prediction. However, these approaches would eliminate range or Doppler information and could introduce negative impact on the classification accuracy. Some et al. [?] processes data from multiple antennas into point clouds, which is not applicable on uni-antenna(?) sensors. Moreover, Wang et al. \cite{wang2016interacting} utilise time–range–Doppler data cube for hand gesture recognition on embedded systems.

%%%

% Some et al. \cite{wang2016interacting} introduce the 3D CNN-LSTM model to radar gesture recognition, but they put minor effort on noise due to property of their sensor and task. However, radar signals the FMCW for whole body activity recognition contain significantly amount of noises []. 

%%%%

Embedded Gaussian non-local block \cite{wang2018non}, considered as a generalization of self-attention \cite{vaswani2017attention}, could improve the performance of both 2D and 3D convolutional neural networks (CNN). It could help the models to focus on important information and capture long-term time information. 


%%%%

% Firstly, a data matrix is reshaped from an array of complex samples, which is received by one antenna. Secondly, the matrix is split on the Short Time axis, based on number of collected frames [], to generate frame sequences. Then, Fast Time fast Fourier transform (FFT) and Slow Time FFT is applied on rows and columns of the each frame to form range-Doppler maps. Meanwhile, Hann window is utilized in FFT to suppress the sidelobe []. Finally, the processed frames are stacked to form 3D time–range–Doppler data cube (range-Doppler map video) as shown in Fig. []. 


%%%
% To capture the semantic dependencies across time, range and Doppler frequencies, the proposed 3D EfficientNet is integrated with the non-local block to further improve the classification performance. 

==> snippets.tex <==
\begin{table}[htbp!]
\centering 
\caption{Results of 2D/3D ResNet/EfficientNet}
\resizebox{.95\columnwidth}{!}{

\begin{tabular}{c|c|ccc}
\hline 
\multirow{3}{*}{Model}& \multirow{3}{*}{\#Parameters}  & \multicolumn{3}{c}{Leave-$n$-antenna-out}  \\
& &\multicolumn{3}{c}{Test Accuracy (\%)} \\
& &$n=1$ & $n=2$ & $n=3$ \\
% $i$ &  $\hat{\mathcal{F}}_{i}$ & $\hat{H}_{i} \times \hat{W}_{i}$ & $\hat{C}_{i}$ & $\hat{L}_{i}$ \\
\hline 
2D ResNet && & &  \\
2D EfficientNet && & &  \\
3D ResNet & & &&  \\
3D EfficientNet && & &  \\
\hline
\end{tabular} \label{tab:results2d3d} 
}
\end{table}



%%%%

\begin{figure}  %子图加并列
\centering
\subfigure[Before]{
\begin{minipage}[b]{0.22\textwidth}
\includegraphics[width=1\textwidth]{fig/zz_plt.png} 
\end{minipage}
}
\subfigure[After]{
\begin{minipage}[b]{0.22\textwidth}
\includegraphics[width=1\textwidth]{fig/ori_plt.png}
\end{minipage}
}
\caption{Range Doppler Map Before/After Processing}
\end{figure}

%%%%% Table 
\begin{table}[htbp!]
\centering 
\caption{Results of Different Number of Non-local Blocks}
% \resizebox{.95\columnwidth}{!}{

\begin{tabular}{cc|cc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Model}} & \multicolumn{2}{|c}{Test Acc (\%)} \\
 &  & $50/50$ & $2/2$ \\
% \multicolumn{2}{c|} { Model } & top-1 & top-5 \\
\midrule
\midrule
\multirow{3}{*} { 3D ResNet-10 } 
& without &  &  \\
& pos. a &  &  \\
& pos. b &  &  \\
\midrule
\multirow{4}{*} { 3D EfficientNet-B0 } 
& without &  &  \\
& pos. a &  &  \\
& pos. b & &  \\
& pos. c & &  \\
\bottomrule
\end{tabular}

\label{tab:resultblocks} 
% }
\end{table}



%%%%

\subsection{Non-local}



%%%%% Table 
\begin{table}[htbp!]
\centering 
\caption{Results of Different Number of Non-local Blocks}
% \resizebox{.95\columnwidth}{!}{

\begin{tabular}{cc|cc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Model}} & \multicolumn{2}{|c}{Test Acc (\%)} \\
 &  & $50/50$ & $2/2$ \\
% \multicolumn{2}{c|} { Model } & top-1 & top-5 \\
\midrule
\midrule
\multirow{3}{*} { 3D ResNet-10 } 
& without &  &  \\
& 1-block &  &  \\
& 5-block &  &  \\
\midrule
\multirow{3}{*} { 3D EfficientNet-B0 } 
& without &  &  \\
& 1-block &  &  \\
& 5-block & &  \\
\bottomrule
\end{tabular}

\label{tab:resultblocks} 
% }
\end{table}



%%%
Generally, we average the results from $6$ independent random shuffle 50\%-50\% splits and $6$ leave-$2$-antenna-out splits on the proposed methods. For the leave-$2$-antenna-out splits,  all the inputs generated from certain $2$ antennas are left for testing while remaining samples  are utilized for training, and thus there are 
$\big(\begin{smallmatrix}
  2 \\
  4 
\end{smallmatrix}\big)=6$  
combinations in total. This approach aims to forbid the information from certain $2$ antennas. Thus, the testing results could partly reveal model performance on unknown FMCW or on FMCW with less antennas.

%%%%
Some et al. [,] utilise wearable radar sensor to detect hand gesture. Their sensor has limited sensing range, closes to the detected hand and validated on consistent background. Hence, the sensor generate relatively clean signals and minor noise elimination should be considered. On the contrary, human activity recognition relatively longer detection range and consequently massive unrelated objects would be involved during sensing. The noises would be revealed on the generated images and thus reduce classification accuracy of the models. Thus, non-local block is introduced to the proposed 3D networks tackle this situation. 

%%%
Inspired by non-local means filter [] for denoising, non-local [] could resolve long-range dependency between pixels with weights. Meanwhile, the utilized embedded Gaussian non-local is a generalized version of self-attention [], which could introduce attentional behavior for the network to focus more on useful areas
% , while neglecting noises. 
Furthermore, the method can naturally interpret temporal information because related components within a video might be presented with long distance and time interval, and the model could interpret their dependency [].  


%%%%
Following (the experiment results from) Wang et al. [], we insert the non-local blocks at relatively deep stages because high-stage non-local blocks consumes less GPU memory and they have similar information abstraction ability with shallow layers, which introduces similar performances. $\{1,5\}$-block non-local are inserted into position \emph{a} or \emph{b} in 3D ResNet-10 as shown in Table \ref{tab:resnet} and inserted into position \emph{a}, \emph{b} or \emph{c} in 3D EfficientNet-B0 as shown in Table \ref{tab:eff}.



%%%%

\begin{table}[htbp!]
\centering 
\caption{Results of Proposed Architectures}
\resizebox{.95\columnwidth}{!}{

\begin{tabular}{c|c|cc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{params} & \multicolumn{2}{c}{Test Acc (\%)} \\
% \multirow{3}{*}{Model}& \multirow{3}{*}{\#Parameters}  & \multicolumn{3}{c}{Leave-$n$-antenna-out}  \\
% & &\multicolumn{3}{c}{Test Accuracy (\%)} \\
 &  & $50/50$ & $2/2$ \\
% $i$ &  $\hat{\mathcal{F}}_{i}$ & $\hat{H}_{i} \times \hat{W}_{i}$ & $\hat{C}_{i}$ & $\hat{L}_{i}$ \\
\midrule
\midrule
2D ResNet-10 &   & &   \\
2D EfficientNet-B0 & & &  \\
\midrule
3D ResNet-10 & & &  \\
3D EfficientNet-B0  & & &  \\
\midrule
3D ResNet-10 + Non-local& & &  \\
3D EfficientNet-B0 + Non-local& & &   \\
\bottomrule
\end{tabular} \label{tab:results2d3d} 
}
\end{table}


%%%%
Radar signals are processed into time–range–Doppler data cube through range-Doppler processing \cite{li2019survey, liu2020real}. Some works further squeeze the cube into time-Doppler maps [?] or time-range [?] maps for prediction. However, these approaches would eliminate range or Doppler information and could introduce negative impact on the classification accuracy. Some et al. [?] processes data from multiple antennas into point clouds, which is not applicable on uni-antenna(?) sensors. Moreover, Wang et al. \cite{wang2016interacting} utilise time–range–Doppler data cube for hand gesture recognition on embedded systems.

%%%

% Some et al. \cite{wang2016interacting} introduce the 3D CNN-LSTM model to radar gesture recognition, but they put minor effort on noise due to property of their sensor and task. However, radar signals the FMCW for whole body activity recognition contain significantly amount of noises []. 

%%%%

Embedded Gaussian non-local block \cite{wang2018non}, considered as a generalization of self-attention \cite{vaswani2017attention}, could improve the performance of both 2D and 3D convolutional neural networks (CNN). It could help the models to focus on important information and capture long-term time information. 


%%%%

% Firstly, a data matrix is reshaped from an array of complex samples, which is received by one antenna. Secondly, the matrix is split on the Short Time axis, based on number of collected frames [], to generate frame sequences. Then, Fast Time fast Fourier transform (FFT) and Slow Time FFT is applied on rows and columns of the each frame to form range-Doppler maps. Meanwhile, Hann window is utilized in FFT to suppress the sidelobe []. Finally, the processed frames are stacked to form 3D time–range–Doppler data cube (range-Doppler map video) as shown in Fig. []. 


%%%
% To capture the semantic dependencies across time, range and Doppler frequencies, the proposed 3D EfficientNet is integrated with the non-local block to further improve the classification performance. 
